Generators and Relations for Un(Z[1/2,i])

Consider the universal gate set for quantum computing consisting of the gates X, CX, CCX, omega^dagger H, and S. All of these gates have matrix entries in the ring Z[1/2,i], the smallest subring of the complex numbers containing 1/2 and i. Amy, Glaudell, and Ross proved the converse, i.e., any unitary matrix with entries in Z[1/2,i] can be realized by a quantum circuit over the above gate set using at most one ancilla. In this paper, we give a finite presentation by generators and relations of U_n(Z[1/2,i]), the group of unitary nxn-matrices with entries in Z[1/2,i].

==> eptcsdata.tex <==
\providecommand{\firstpage}{145}
\providecommand{\publicationstatus}{M. Backens, C. Heunen (Eds.): Quantum Physics and Logic (QPL) 2021\\
EPTCS 343, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.343.8}{10.4204/EPTCS.343.8}}
\pdfoutput=1

